Mining Supervision for Dynamic Regions in Self-Supervised Monocular Depth Estimation

This paper focuses on self-supervised monocular depth estimation in dynamic scenes trained on monocular videos. Existing methods jointly estimate pixel-wise depth and motion, relying mainly on an image reconstruction loss. Dynamic regions1 remain a critical challenge for these methods due to the inherent ambiguity in depth and motion estimation, resulting in inaccurate depth estimation. This paper proposes a self-supervised training framework exploiting pseudo depth labels for dynamic regions from training data. The key contribution of our framework is to decouple depth estimation for static and dynamic regions of images in the training data. We start with an unsupervised depth estimation approach, which provides reliable depth estimates for static regions and motion cues for dynamic regions and allows us to extract moving object information at the instance level. In the next stage, we use an object network to estimate the depth of those moving objects assuming rigid motions. Then, we propose a new scale alignment module to address the scale ambiguity between estimated depths for static and dynamic regions. We can then use the depth labels generated to train an end-to-end depth estimation network and improve its performance. Extensive experiments on the Cityscapes and KITTI datasets show that our self-training strategy consistently outperforms existing self/unsupervised depth estimation methods.

==> main/5_limitations.tex <==

\section{Limitations}

==> old_table/comparision_with_SOTA.tex <==


\begin{table*}[h]
\scriptsize
\centering
\begin{tabular}{|c|c|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Method} &
\multirow{2}{*}{Dataset} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sematic\\ prior\end{tabular}} &
  \multicolumn{3}{c|}{Dynamic region} &
  \multicolumn{3}{c|}{Static region} &
  \multicolumn{3}{c|}{All region} \\ \cline{4-12} 
   &
   &
   & 
  \multicolumn{1}{c|}{Abs Rel} &
  \multicolumn{1}{c|}{Sq Rel} &
  $\delta < 1.25$ &
  \multicolumn{1}{c|}{Abs Rel} &
  \multicolumn{1}{c|}{Sq Rel} &
  $\delta < 1.25$ &
  \multicolumn{1}{c|}{Abs Rel} &
  \multicolumn{1}{c|}{Sq Rel} &
  $\delta < 1.25$ \\ \hline \hline
Monodepth2* \cite{godard2019digging} &
    % C   &
\multirow{5}{*}{C}
        &
        &
  0.286 &
  6.036 &
  0.716 &
  0.119 &
  1.461 &
  0.877 &
  0.127 &
  1.678 &
  0.872 \\
Li \textit{et al.}* \cite{li2021unsupervised} & 
   &
   &
  0.188 &
  1.654 &
  0.735 &
  0.118 &
  1.198 &
  0.835 &
  0.119 &
  1.186 &
  0.833 \\
InstaDM \cite{lee2021learning} & 
    &
  \checkmark &
  0.189 &
  2.538 &
  0.795 &
  0.102 &
  1.058 &
  0.895 &
  0.106 &
  1.104 &
  0.890 \\
RMDepth \cite{hui2022rm} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  0.100 &
  0.839 &
  0.895 \\

DaCNN \cite{han2023self} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  0.113 &
  1.380 &
  0.888 \\

% % ManyDepth \cite{watson2021temporal} & 
% %     &
% %    &
% %   \checkmark &
% %   0.314 &
% %   5.127 &
% %   0.571 &
% %   0.106 &
% %   1.061 &
% %   0.885 &
% %   0.114 &
% %   1.193 &
% %   0.875 \\
% % DynamicDepth \cite{feng2022disentangling} & 
% %     &
% %   \checkmark &
% %   \checkmark &
% %   0.236 &
% %   3.478 &
% %   0.703 &
% %   0.099 &
% %   0.942 &
% %   0.896 &
% %   0.103 &
% %   1.000 &
% %   0.895 \\
\hline 


ResNet18 \cite{gordon2019depth}   + Ours & 
\multirow{4}{*}{C}
   &
   &
  \textbf{\underline{0.107}} &
  \underline{0.784} &
  \textbf{\underline{0.907}} &
  \underline{0.093} &
  \underline{0.961} &
  \underline{0.907} &
  \underline{0.094} &
  0.931 &
  \underline{0.906} \\
PackNet \cite{guizilini20203d} + Ours & 
   &
   &
  \underline{0.112} &
  \underline{0.703} &
  \underline{0.890} &
  \underline{0.090} &
  \underline{0.858} &
  \underline{0.909} &
  \underline{0.091} &
  \underline{0.831} &
  \underline{0.908} \\
DiffNet \cite{zhou2021self} + Ours & 
   &
   &
  \underline{0.113} &
  \textbf{\underline{0.657}} &
  \underline{0.889} &
  \underline{0.083} &
  \underline{0.775} &
  \underline{0.919} &
  \underline{0.085} &
  \underline{0.753} &
  \underline{0.916} \\
BrNet \cite{han2022brnet} + Ours & 
   &
   &
  \underline{0.119} &
  \underline{0.670} &
  \underline{0.872} &
  \textbf{\underline{0.080}} &
  \textbf{\underline{0.736}} &
  \textbf{\underline{0.922}} &
  \textbf{\underline{0.084}} &
  \textbf{\underline{0.722}} &
  \textbf{\underline{0.918}} \\
% ManyDepth \cite{watson2021temporal} +   Ours & 
%     &
%    & 
%   \checkmark &
%   \underline{0.122} &
%   \underline{0.819} &
%   \underline{0.871} &
%   \underline{0.084} &
%   \underline{0.812} &
%   \underline{0.918} &
%   \underline{0.087} &
%   \underline{0.793} &
%   \underline{0.915} \\
  \hline \hline 

PackNet \cite{guizilini20203d} & 
\multirow{5}{*}{K}
   &
   &
   0.213 &
   2.820 &
   0.762 &
   0.108 &
   0.814 &
   0.883 &
   0.110 &
   0.834 &
   0.881 \\  

DiffNet \cite{zhou2021self} & 
   &
   &
   0.177 &
   2.072 &
   0.930 &
   0.101 &
   0.743 &
   \textbf{0.899} &
   0.102 &
   0.753 &
   0.897 \\  

BrNet* \cite{han2022brnet} & 
   &
   &
   0.183 &
   1.715 &
   0.760 &
   0.104 &
   0.702 &
   0.885 &
   0.106 &
   0.711 &
   0.884 \\  
RMDepth \cite{hui2022rm} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
   {0.108} &
   {0.710} &
   {0.884} \\ 
DaCNN \cite{han2023self} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
   \textbf{0.099} &
   \textbf{0.661} &
   \textbf{0.897} \\   
\hline
DiffNet \cite{zhou2021self} + Ours & 
\multirow{4}{*}{K}
   &
   &
   \underline{0.158}&
   \underline{1.468} &
   \underline{0.838} &
   0.101 &
   \underline{0.687} &
   0.894 &
   0.102 &
   0.693 &
   0.892 \\  
% # [0.1, 0.662, 4.473, 0.179, 0.894, 0.965, 0.983]
% # [0.099, 0.658, 4.471, 0.176, 0.895, 0.966, 0.984]
% # [0.143, 1.191, 5.095, 0.268, 0.845, 0.911, 0.941]
DiffNet \cite{zhou2021self} + Ours & 
    & \checkmark
   &
   \textbf{\underline{0.143}} &
   \textbf{\underline{1.191}} &
   \textbf{\underline{0.845}} & 
   \textbf{\underline{0.099}} &
   \textbf{\underline{0.658}} &
   0.895 &
   0.100 &
   0.662 &
   0.894 \\ 
BrNet \cite{han2022brnet} + Ours & 
    &
   &
   \underline{0.160} &
   \underline{1.273} &
   \underline{0.812} &
   0.103 &
   \underline{0.690} &
   \textbf{0.889} &
   0.103 &
   0.692 &
   0.888 \\  

BrNet \cite{han2022brnet} + Ours & 
    & \checkmark
   &
   \underline{0.162} &
   \underline{1.207} &
   \underline{0.812} &
   0.102 &
   \underline{0.673} &
   \textbf{0.889} &
   0.103 &
   0.675 &
   0.888 \\  
\hline
\end{tabular}
\caption{Comparison between the models trained with our method and previous works on Cityscapes (C) and Kitti (K) dataset. The best results are in \textbf{bold}. Additionally, the performance of our methods is \underline{underlined} if it is better than all previous works. (*) indicates results reproduced using the official code. All methods are trained on monocular videos.}
\vspace{-5mm}
\label{Tab:result_comparision_to_SOTA}
\end{table*}

==> old_table/stage_wise_training.tex <==

\begin{table*}[h]
\scriptsize
\centering
\label{Tab:result_stage_wise_training}
\begin{tabular}{|c|c|c|c|ccc|ccc|ccc|}
\hline &  &   &   & \multicolumn{3}{c|}{Dynamic region}   & \multicolumn{3}{c|}{Static region}                              & \multicolumn{3}{c|}{All region}                                                         \\ \cline{5-13}
\multirow{-2}{*}{Backbone} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Pixel \\ motion\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Pseudo\\ depth\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Sematic\\ prior\end{tabular}} & \multicolumn{1}{c|}{Abs Rel} & \multicolumn{1}{c|}{Sq Rel} & $\delta < 1.25$ & \multicolumn{1}{c|}{Abs Rel} & \multicolumn{1}{c|}{Sq Rel} & $\delta < 1.25$ & \multicolumn{1}{c|}{Abs Rel} & \multicolumn{1}{c|}{Sq Rel} & $\delta < 1.25$ \\ \hline
\hline

% Resnet18 \cite{gordon2019depth}

\multirow{4}{*}{Resnet18 \cite{gordon2019depth}} &   &   &   & 0.352 & 11.169 & 0.858 & 0.118 & 1.362 & 0.862 & 0.127 & 1.743 & 0.722 \\

& \checkmark &   &   & 0.144 & 1.650 & 0.898 & 0.095 & 0.986 & 0.900 & 0.097 & 0.982 & 0.854 \\

& \checkmark & \checkmark &   & \underline{0.107} & \underline{0.784} & \textbf{0.906} & \underline{0.093} & \underline{0.961} & \textbf{0.907} & \underline{0.094} & \underline{0.931} & \underline{0.907} \\

& \checkmark & \checkmark & \checkmark & \textbf{0.100} & \textbf{0.647} & \underline{0.903} & \textbf{0.091} & \textbf{0.931} & \underline{0.904} & \textbf{0.092} & \textbf{0.895} & \textbf{0.911} \\
\hline
\hline
% 
\multirow{4}{*}{Packnet \cite{guizilini20203d}}
&   &   &   & 0.182 & 2.667 & 0.891 & 0.104 & 1.167 & 0.894 & 0.108 & 1.210 & 0.813 \\
& \checkmark &   &   & 0.132 & 0.987 & \underline{0.906} & 0.091 & 0.861 & \underline{0.908} & 0.093 & 0.844 & 0.857 \\
& \checkmark & \checkmark &   & \underline{0.112} & \underline{0.703} & \textbf{0.908} & \underline{0.090} & \textbf{0.858} & \textbf{0.909} & \underline{0.091} & \underline{0.831} & \underline{0.890} \\
& \checkmark & \checkmark & \checkmark & \textbf{0.104} & \textbf{0.666} & \textbf{0.908} & \textbf{0.089} & \underline{0.859} & \underline{0.908} & \textbf{0.090} & \textbf{0.830} & \textbf{0.901} \\
\hline
\hline

 \multirow{4}{*}{DiffNet \cite{zhou2021self} } &   &   &   & 0.233 & 4.369 & 0.893 & 0.103 & 1.109 & 0.896 & 0.107 & 1.187 & 0.771 \\
& \checkmark &   &   & 0.152 & 1.646 & 0.912 & 0.087 & 0.831 & 0.917 & 0.090 & 0.833 & 0.828 \\
& \checkmark & \checkmark &   & \underline{0.113} & \textbf{0.657} & \underline{0.916} & \underline{0.083} & \textbf{0.775} & \underline{0.919} & \underline{0.085} & \textbf{0.753} & \underline{0.889} \\
& \checkmark & \checkmark & \checkmark & \textbf{0.105} & \underline{0.692} & \textbf{0.919} & \textbf{0.082} & \underline{0.781} & \textbf{0.921} & \textbf{0.083} & \underline{0.757} & \textbf{0.893} \\
\hline
\hline

 \multirow{4}{*}{BrNet \cite{han2022brnet}}  &   &    &   & 0.224 & 3.440 & 0.883 & 0.105 & 1.052 & 0.889 & 0.106 & 1.124 & 0.707 \\
& \checkmark &   &   &  0.168 & 2.041 & 0.914 & \underline{0.082} & 0.747 & 0.920 & 0.087 & 0.780 & 0.809 \\
& \checkmark & \checkmark &   &  \underline{0.119} & \underline{0.670} & \underline{0.918} & \textbf{0.080} & \underline{0.736} & \underline{0.922} & \underline{0.084} & \underline{0.722} & \underline{0.872} \\
& \checkmark & \checkmark & \checkmark &  \textbf{0.106} & \textbf{0.577} & \textbf{0.921} & \textbf{0.080} & \textbf{0.717} & \textbf{0.923} & \textbf{0.081} & \textbf{0.696} & \textbf{0.892} \\
\hline


% \multirow{4}{*}{ManyDepth \cite{watson2021temporal}}
% &   &   &  \checkmark & 0.314 & 5.127 & 0.875 & 0.106 & 1.061 & 0.885 & 0.114 & 1.193 & 0.571 \\
% & \checkmark &   &  \checkmark & 0.157 & 1.393 & 0.911 & \underline{0.087} & 0.824 & 0.916 & 0.091 & 0.825 & 0.807 \\
% & \checkmark & \checkmark &   & \checkmark\underline{0.122} & \underline{0.819} & \underline{0.915} & \textbf{0.084} & \underline{0.812} & \underline{0.918} & \underline{0.087} & \underline{0.793} & \underline{0.871} \\
% & \checkmark & \checkmark & \checkmark & \checkmark\textbf{0.109} & \textbf{0.709} & \textbf{0.918} & \textbf{0.084} & \textbf{0.810} & \textbf{0.919} & \textbf{0.086} & \textbf{0.785} & \textbf{0.898} \\

% \hline

\end{tabular}
\caption{Results of training different depth estimation networks backbone under different settings. For each backbone, the best results are in \textbf{bold}, the second best are \underline{underlined}. \noindent\textbf{With pixel wise:} The model is trained in our first stage only. 
\noindent\textbf{With pixel motion and pseudo depth:} Our fully self-supervised pipeline is applied to train the model.   
\noindent\textbf{With sematic prior:} Objects and ground masks are produced by a pre-trained segmentation model \cite{zou2023segment} instead of the self-supervised ones.}
\label{Tab:result_stage_wise_training}
\end{table*}



\begin{table*}[h]
\scriptsize
\centering
\begin{tabular}{|c|c|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Method} &
\multirow{2}{*}{Dataset} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sematic\\ prior\end{tabular}} &
  \multicolumn{3}{c|}{Dynamic region} &
  \multicolumn{3}{c|}{Static region} &
  \multicolumn{3}{c|}{All region} \\ \cline{4-12} 
   &
   &
   & 
  \multicolumn{1}{c|}{Abs Rel} &
  \multicolumn{1}{c|}{Sq Rel} &
  $\delta < 1.25$ &
  \multicolumn{1}{c|}{Abs Rel} &
  \multicolumn{1}{c|}{Sq Rel} &
  $\delta < 1.25$ &
  \multicolumn{1}{c|}{Abs Rel} &
  \multicolumn{1}{c|}{Sq Rel} &
  $\delta < 1.25$ \\ \hline \hline
Monodepth2* \cite{godard2019digging} &
    % C   &
\multirow{5}{*}{C}
        &
        &
  0.286 &
  6.036 &
  0.716 &
  0.119 &
  1.461 &
  0.877 &
  0.127 &
  1.678 &
  0.872 \\
Li \textit{et al.}* \cite{li2021unsupervised} & 
   &
   &
  0.188 &
  1.654 &
  0.735 &
  0.118 &
  1.198 &
  0.835 &
  0.119 &
  1.186 &
  0.833 \\
InstaDM \cite{lee2021learning} & 
    &
  \checkmark &
  0.189 &
  2.538 &
  0.795 &
  0.102 &
  1.058 &
  0.895 &
  0.106 &
  1.104 &
  0.890 \\
RMDepth \cite{hui2022rm} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  0.100 &
  0.839 &
  0.895 \\

DaCNN \cite{han2023self} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  0.113 &
  1.380 &
  0.888 \\

% % ManyDepth \cite{watson2021temporal} & 
% %     &
% %    &
% %   \checkmark &
% %   0.314 &
% %   5.127 &
% %   0.571 &
% %   0.106 &
% %   1.061 &
% %   0.885 &
% %   0.114 &
% %   1.193 &
% %   0.875 \\
% % DynamicDepth \cite{feng2022disentangling} & 
% %     &
% %   \checkmark &
% %   \checkmark &
% %   0.236 &
% %   3.478 &
% %   0.703 &
% %   0.099 &
% %   0.942 &
% %   0.896 &
% %   0.103 &
% %   1.000 &
% %   0.895 \\
\hline 


ResNet18 \cite{gordon2019depth}   + Ours & 
\multirow{4}{*}{C}
   &
   &
  \textbf{\underline{0.107}} &
  \underline{0.784} &
  \textbf{\underline{0.907}} &
  \underline{0.093} &
  \underline{0.961} &
  \underline{0.907} &
  \underline{0.094} &
  0.931 &
  \underline{0.906} \\
PackNet \cite{guizilini20203d} + Ours & 
   &
   &
  \underline{0.112} &
  \underline{0.703} &
  \underline{0.890} &
  \underline{0.090} &
  \underline{0.858} &
  \underline{0.909} &
  \underline{0.091} &
  \underline{0.831} &
  \underline{0.908} \\
DiffNet \cite{zhou2021self} + Ours & 
   &
   &
  \underline{0.113} &
  \textbf{\underline{0.657}} &
  \underline{0.889} &
  \underline{0.083} &
  \underline{0.775} &
  \underline{0.919} &
  \underline{0.085} &
  \underline{0.753} &
  \underline{0.916} \\
BrNet \cite{han2022brnet} + Ours & 
   &
   &
  \underline{0.119} &
  \underline{0.670} &
  \underline{0.872} &
  \textbf{\underline{0.080}} &
  \textbf{\underline{0.736}} &
  \textbf{\underline{0.922}} &
  \textbf{\underline{0.084}} &
  \textbf{\underline{0.722}} &
  \textbf{\underline{0.918}} \\
% ManyDepth \cite{watson2021temporal} +   Ours & 
%     &
%    & 
%   \checkmark &
%   \underline{0.122} &
%   \underline{0.819} &
%   \underline{0.871} &
%   \underline{0.084} &
%   \underline{0.812} &
%   \underline{0.918} &
%   \underline{0.087} &
%   \underline{0.793} &
%   \underline{0.915} \\
  \hline \hline 

PackNet \cite{guizilini20203d} & 
\multirow{5}{*}{K}
   &
   &
   0.213 &
   2.820 &
   0.762 &
   0.108 &
   0.814 &
   0.883 &
   0.110 &
   0.834 &
   0.881 \\  

DiffNet \cite{zhou2021self} & 
   &
   &
   0.177 &
   2.072 &
   0.930 &
   0.101 &
   0.743 &
   \textbf{0.899} &
   0.102 &
   0.753 &
   0.897 \\  

BrNet* \cite{han2022brnet} & 
   &
   &
   0.183 &
   1.715 &
   0.760 &
   0.104 &
   0.702 &
   0.885 &
   0.106 &
   0.711 &
   0.884 \\  
RMDepth \cite{hui2022rm} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
   {0.108} &
   {0.710} &
   {0.884} \\ 
DaCNN \cite{han2023self} & 
   &
   &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
  \textendash &
   \textbf{0.099} &
   \textbf{0.661} &
   \textbf{0.897} \\   
\hline
DiffNet \cite{zhou2021self} + Ours & 
\multirow{4}{*}{K}
   &
   &
   \underline{0.158}&
   \underline{1.468} &
   \underline{0.838} &
   0.101 &
   \underline{0.687} &
   0.894 &
   0.102 &
   0.693 &
   0.892 \\  
% # [0.1, 0.662, 4.473, 0.179, 0.894, 0.965, 0.983]
% # [0.099, 0.658, 4.471, 0.176, 0.895, 0.966, 0.984]
% # [0.143, 1.191, 5.095, 0.268, 0.845, 0.911, 0.941]
DiffNet \cite{zhou2021self} + Ours & 
    & \checkmark
   &
   \textbf{\underline{0.143}} &
   \textbf{\underline{1.191}} &
   \textbf{\underline{0.845}} & 
   \textbf{\underline{0.099}} &
   \textbf{\underline{0.658}} &
   0.895 &
   0.100 &
   0.662 &
   0.894 \\ 
BrNet \cite{han2022brnet} + Ours & 
    &
   &
   \underline{0.160} &
   \underline{1.273} &
   \underline{0.812} &
   0.103 &
   \underline{0.690} &
   \textbf{0.889} &
   0.103 &
   0.692 &
   0.888 \\  

BrNet \cite{han2022brnet} + Ours & 
    & \checkmark
   &
   \underline{0.162} &
   \underline{1.207} &
   \underline{0.812} &
   0.102 &
   \underline{0.673} &
   \textbf{0.889} &
   0.103 &
   0.675 &
   0.888 \\  
\hline
\end{tabular}
\caption{Comparison between the models trained with our method and previous works on Cityscapes (C) and Kitti (K) dataset. The best results are in \textbf{bold}. Additionally, the performance of our methods is \underline{underlined} if it is better than all previous works. (*) indicates results reproduced using the official code. All methods are trained on monocular videos.}
\vspace{-5mm}
\label{Tab:result_comparision_to_SOTA}
\end{table*}
